Token-Scaled Logit Distillation for Ternary Weight Generative Language Models

Generative Language Models (GLMs) have shown impressive performance in tasks such as text generation, understanding, and reasoning. However, the large model size poses challenges for practical deployment. To solve this problem, Quantization-Aware Training (QAT) has become increasingly popular. However, current QAT methods for generative models have resulted in a noticeable loss of accuracy. To counteract this issue, we propose a novel knowledge distillation method specifically designed for GLMs. Our method, called token-scaled logit distillation, prevents overfitting and provides superior learning from the teacher model and ground truth. This research marks the first evaluation of ternary weight quantization-aware training of large-scale GLMs with less than 1.0 degradation in perplexity and achieves enhanced accuracy in tasks like common-sense QA and arithmetic reasoning as well as natural language understanding. Our code is available at https://github.com/aiha-lab/TSLD.

==> Tables/table2.tex <==
\begin{table}[htbp]
\footnotesize
\centering
\begin{tabular}{c|c|c|cccc}
\toprule
\multirow{2}{*}{Task}                       & \multirow{2}{*}{Precision}                  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Optimization\\ Method\end{tabular}} & \multicolumn{2}{c|}{2.7B}            & \multicolumn{2}{c}{6.7B} \\ \cline{4-7} 
                                            &                                             &                         & Accuracy & \multicolumn{1}{c|}{PPL}  & Accuracy      & PPL      \\ \toprule
\multicolumn{1}{c|}{\multirow{4}{*}{GSM8K}} & \multicolumn{2}{c|}{FP32 baseline}                                    & 20.39    & \multicolumn{1}{c|}{2.07} & 22.52         & 1.89     \\ \cmidrule{2-7} 
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{3}{*}{W2A32}} & Logit~\cite{QuantGPT}     & 20.02    & \multicolumn{1}{c|}{\textbf{2.03}} & 21.08          & \textbf{1.93}     \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & Logit+GT        & 19.56    & \multicolumn{1}{c|}{2.12} & 18.35         & 2.02     \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & TSLD                    & \textbf{20.24}    & \multicolumn{1}{c|}{\textbf{2.03}} & \textbf{24.49}         & 2.14     \\ \toprule
\end{tabular}
\caption{Accuracy and evaluation perplexity of each methods in GSM8K on OPT models}
\label{table2}
\end{table}\begin{table}[htbp]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{c|c|cc|cc|cc|cc}
\toprule
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Precision\\ (Size)\end{tabular}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}QAT KD\\ Method\end{tabular}}} & \multicolumn{2}{c|}{CoLA}       & \multicolumn{2}{c|}{MRPC}       & \multicolumn{2}{c|}{SST-2}      & \multicolumn{2}{c}{RTE}        \\ \cmidrule{3-10}
&& ACC (↑)        & PPL (↓)       & ACC (↑)        & PPL (↓)       & ACC (↑)        & PPL (↓)       & ACC (↑)        & PPL (↓)       \\ \midrule
\multicolumn{2}{c|}{OPT-1.3B FP16 (2.5 GB)}                                                                                   & 61.03          & 1.34          & 81.92          & 2.58          & 94.26          & 2.00          & 76.53          & 3.94          \\ \midrule
% \multicolumn{1}{c|}{W8A16} & \multicolumn{1}{c|}{GT} & & & & & & & &  \\ \midrule
\multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}W4A16\\ (761.9 MB)\end{tabular}}}       & GPTQ-CW                                                                   & 54.61          & \textbf{1.36}          &   80.14   &  \textbf{2.43}   & \textbf{95.07}    &  \textbf{2.02}      & 56.32           & \textbf{3.96}          \\ 
 & AWQ-CW                                                                   & 13.63          & 1.45          & 66.42         & 3.49          & 94.26          & \textbf{2.02}          & 54.51           & 4.72          \\  \cmidrule{2-10}

& Logit [20]                                                                   & 50.76 {\color{gray}\scriptsize±2.35}         & 1.36          & 81.94  {\color{gray}\scriptsize±1.48}        & 2.62          & 93.57  {\color{gray}\scriptsize±0.23}        & 2.09          & 75.23  {\color{gray}\scriptsize±0.83}          & 4.34          \\
                               & GT+Logit                                                                  & 54.07 {\color{gray}\scriptsize±0.34}         & \textbf{1.34} & 83.17 {\color{gray}\scriptsize±0.51}         & 2.60          & 93.34 {\color{gray}\scriptsize±0.22}         & 2.11          & 75.31 {\color{gray}\scriptsize±1.07}         & 4.09          \\
                               & TSLD                                                                      & \textbf{56.33} {\color{gray}\scriptsize±0.98} & \textbf{1.34} & \textbf{83.33} {\color{gray}\scriptsize±1.22} & \textbf{2.52} & 94.05 {\color{gray}\scriptsize±0.19} & 2.04 & \textbf{75.97} {\color{gray}\scriptsize±0.31} & \textbf{4.05} \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}W2A16\\ (473.2 MB)\end{tabular}}}         & Logit [20]                                                                    & 48.72 {\color{gray}\scriptsize±2.68}         & 1.37          & 81.62 {\color{gray}\scriptsize±0.62}         & 2.79          & 93.08 {\color{gray}\scriptsize±0.35}         & 2.11          & 74.15 {\color{gray}\scriptsize±1.36}         & 4.72          \\
                               & GT+Logit                                                                  & 50.10  {\color{gray}\scriptsize±1.38}        & \textbf{1.34} & 82.10 {\color{gray}\scriptsize±0.99}         & 2.65          & 92.77 {\color{gray}\scriptsize±0.28}        & 2.14          & 73.79 {\color{gray}\scriptsize±1.16}         & 4.44          \\
                               & TSLD                                                                      & \textbf{54.47} {\color{gray}\scriptsize±1.47} & \textbf{1.34} & \textbf{82.20} {\color{gray}\scriptsize±0.94} & \textbf{2.63} & \textbf{93.92} {\color{gray}\scriptsize±0.29} & \textbf{2.06} & \textbf{75.31} {\color{gray}\scriptsize±0.54} & \textbf{4.36} \\ \toprule
\end{tabular}
}
\caption{\small Accuracy (ACC) and Perplexity (PPL) results of the OPT-1.3B model fine-tuned on the NLU (GLUE) with different QAT-KD methods. The results are based on five random seed tests, and the model size for each precision is indicated in parentheses next to the precision. GPTQ-CW and AWQ-CW denote the latest SOTA PTQ methodology, and we apply quantization on an output channel-wise basis (CW) }
\vskip-0.2in
\label{tab:nlu}
\end{table}
